Trade-offs of Dynamic Control Structure in Human-swarm Systems

Swarm robotics is a study of simple robots that exhibit complex behaviour only by interacting locally with other robots and their environment. The control in swarm robotics is mainly distributed whereas centralised control is widely used in other fields of robotics. Centralised and decentralised control strategies both pose a unique set of benefits and drawbacks for the control of multi-robot systems. While decentralised systems are more scalable and resilient, they are less efficient compared to the centralised systems and they lead to excessive data transmissions to the human operators causing cognitive overload. We examine the trade-offs of each of these approaches in a human-swarm system to perform an environmental monitoring task and propose a flexible hybrid approach, which combines elements of hierarchical and decentralised systems. We find that a flexible hybrid system can outperform a centralised system (in our environmental monitoring task by 19.2%) while reducing the number of messages sent to a human operator (here by 23.1%). We conclude that establishing centralisation for a system is not always optimal for performance and that utilising aspects of centralised and decentralised systems can keep the swarm from hindering its performance.

==> extratable.tex <==
\begin{table}[]
\begin{tabular}{|l|ccc|ccc|}
\hline
\multirow{2}{*}{}           & \multicolumn{3}{c|}{{\textbf{Hybrid}}}                                           & \multicolumn{3}{c|}{{\textbf{Hierarchical}}}                                     \\ \cline{2-7} 
                            & \multicolumn{1}{c|}{\textbf{25}} & \multicolumn{1}{c|}{\textbf{100}} & \textbf{1000} & \multicolumn{1}{c|}{\textbf{25}} & \multicolumn{1}{c|}{\textbf{100}} & \textbf{1000} \\ \hline
\textbf{Mean time w/ trees} & \multicolumn{1}{c|}{7933s}       & \multicolumn{1}{c|}{5636s}        & 1625s         & \multicolumn{1}{c|}{7167s}       & \multicolumn{1}{c|}{6020s}        & 2492s         \\ \hline
\textbf{Mean \# of trees}   & \multicolumn{1}{c|}{1.83}        & \multicolumn{1}{c|}{1.45}         & 1.10          & \multicolumn{1}{c|}{1.83}        & \multicolumn{1}{c|}{1.47}         & 1.08          \\ \hline
\textbf{Mean tree size}     & \multicolumn{1}{c|}{6.27}        & \multicolumn{1}{c|}{7.05}         & 6.19          & \multicolumn{1}{c|}{6.01}        & \multicolumn{1}{c|}{6.93}         & 5.17          \\ \hline
\textbf{Mean max tree size} & \multicolumn{1}{c|}{17.3}        & \multicolumn{1}{c|}{22.8}         & 9.2           & \multicolumn{1}{c|}{17.6}        & \multicolumn{1}{c|}{21.8}         & 11.0          \\ \hline
\end{tabular}
\caption{Statistics of trees formed over the course of a run for both the hybrid and hierarchical approaches with swarm sizes of 25, 100 and 1000 agents.}
\end{table}
